Reqomp: Space-constrained Uncomputation for Quantum Circuits

Quantum circuits must run on quantum computers with tight limits on qubit and gate counts. To generate circuits respecting both limits, a promising opportunity is exploiting uncomputation to trade qubits for gates. We present Reqomp, a method to automatically synthesize correct and efficient uncomputation of ancillae while respecting hardware constraints. For a given circuit, Reqomp can offer a wide range of trade-offs between tightly constraining qubit count or gate count. Our evaluation demonstrates that Reqomp can significantly reduce the number of required ancilla qubits by up to 96%. On 80% of our benchmarks, the ancilla qubits required can be reduced by at least 25% while never incurring a gate count increase beyond 28%.

==> figures/app_sq_correct_eager.tex <==

\def\tikzRowSepDefault{2mm}
\def\tikzColumnSepDefault{0.9mm}
\def\tikzWireLeftDefault{0.7cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-ctrl] (i-X-a-0) {}; &
	\node[style=circuit-ctrl] (i-X-b-0) {}; &
	\node[style=circuit-gate] (i-X-i-0) {$X$}; &
	\node[style=circuit-ctrl] (i-X-b-1) {}; &
	\node[style=circuit-gate] (i-X-i-1) {$X$}; &
	\node[style=circuit-ctrl] (i-X-a-1) {}; &
	\node[style=circuit-noop] (i-6) {}; &
	\node[style=circuit-noop] (i-7) {}; &
	\node[style=circuit-noop] (i-8) {}; &
	\node[style=circuit-ctrl] (i-X-a-4) {}; &
	\node[style=circuit-gate] (i-X-i-2) {$X$}; &
	\node[style=circuit-ctrl] (i-X-b-2) {}; &
	\node[style=circuit-gate] (i-X-i-3) {$X$}; &
	\node[style=circuit-ctrl] (i-X-b-3) {}; &
	\node[style=circuit-ctrl] (i-X-a-5) {}; \\

	\node[style=circuit-gate] (a-X-a-0) {$X$}; &
	\node[style=circuit-noop] (a-1) {}; &
	\node[style=circuit-noop] (a-2) {}; &
	\node[style=circuit-ctrl] (a-X-b-1) {}; &
	\node[style=circuit-noop] (a-4) {}; &
	\node[style=circuit-gate] (a-X-a-1) {$X$}; &
	\node[style=circuit-gate] (a-X-a-2) {$X$}; &
	\node[style=circuit-ctrl] (a-X-r-0) {}; &
	\node[style=circuit-gate] (a-X-a-3) {$X$}; &
	\node[style=circuit-gate] (a-X-a-4) {$X$}; &
	\node[style=circuit-noop] (a-10) {}; &
	\node[style=circuit-ctrl] (a-X-b-2) {}; &
	\node[style=circuit-noop] (a-12) {}; &
	\node[style=circuit-noop] (a-13) {}; &
	\node[style=circuit-gate] (a-X-a-5) {$X$}; \\

	\node[style=circuit-noop] (b-0) {}; &
	\node[style=circuit-gate] (b-X-b-0) {$X$}; &
	\node[style=circuit-noop] (b-2) {}; &
	\node[style=circuit-gate] (b-X-b-1) {$X$}; &
	\node[style=circuit-noop] (b-4) {}; &
	\node[style=circuit-noop] (b-5) {}; &
	\node[style=circuit-ctrl] (b-X-a-2) {}; &
	\node[style=circuit-noop] (b-7) {}; &
	\node[style=circuit-ctrl] (b-X-a-3) {}; &
	\node[style=circuit-noop] (b-9) {}; &
	\node[style=circuit-noop] (b-10) {}; &
	\node[style=circuit-gate] (b-X-b-2) {$X$}; &
	\node[style=circuit-noop] (b-12) {}; &
	\node[style=circuit-gate] (b-X-b-3) {$X$}; &
	\node[style=circuit-noop] (b-14) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-noop] (r-3) {}; &
	\node[style=circuit-noop] (r-4) {}; &
	\node[style=circuit-noop] (r-5) {}; &
	\node[style=circuit-noop] (r-6) {}; &
	\node[style=circuit-gate] (r-X-r-0) {$X$}; &
	\node[style=circuit-noop] (r-8) {}; &
	\node[style=circuit-noop] (r-9) {}; &
	\node[style=circuit-noop] (r-10) {}; &
	\node[style=circuit-noop] (r-11) {}; &
	\node[style=circuit-noop] (r-12) {}; &
	\node[style=circuit-noop] (r-13) {}; &
	\node[style=circuit-noop] (r-14) {}; \\
};
% COORDINATES
% i
\coordinate[left =\tikzWireLeft of i-X-a-0.center] (i-left);
\coordinate[right=\tikzWireRight of i-X-a-5.center] (i-right);

% a
\coordinate[left =\tikzWireLeft of a-X-a-0.center] (a-left);
\coordinate[right=\tikzWireRight of a-X-a-5.center] (a-right);

% b
\coordinate[left =\tikzWireLeft of b-0.center] (b-left);
\coordinate[right=\tikzWireRight of b-14.center] (b-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-14.center] (r-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (i-left) -- (i-right);
	\draw[-] (a-left) -- (a-right);
	\draw[-] (b-left) -- (b-right);
	\draw[-] (r-left) -- (r-right);

	% controls
	\draw[-] (i-X-a-0) -- (a-X-a-0);
	\draw[-] (i-X-b-0) -- (b-X-b-0);
	\draw[-] (i-X-b-1) -- (b-X-b-1);
	\draw[-] (a-X-b-1) -- (b-X-b-1);
	\draw[-] (i-X-a-1) -- (a-X-a-1);
	\draw[-] (b-X-a-2) -- (a-X-a-2);
	\draw[-] (a-X-r-0) -- (r-X-r-0);
	\draw[-] (b-X-a-3) -- (a-X-a-3);
	\draw[-] (i-X-a-4) -- (a-X-a-4);
	\draw[-] (i-X-b-2) -- (b-X-b-2);
	\draw[-] (a-X-b-2) -- (b-X-b-2);
	\draw[-] (i-X-b-3) -- (b-X-b-3);
	\draw[-] (i-X-a-5) -- (a-X-a-5);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(i-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$i$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(a-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_0$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(b-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_1$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};



==> figures/app_sq_incorrect_eager.tex <==

\def\tikzRowSepDefault{2mm}
\def\tikzColumnSepDefault{0.9mm}
\def\tikzWireLeftDefault{0.7cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-ctrl] (i-X-a-0) {}; &
	\node[style=circuit-ctrl] (i-X-b-0) {}; &
	\node[style=circuit-gate] (i-X-i-0) {$X$}; &
	\node[style=circuit-ctrl] (i-X-b-1) {}; &
	\node[style=circuit-ctrl] (i-X-a-1) {}; &
	\node[style=circuit-noop] (i-5) {}; &
	\node[style=circuit-noop] (i-6) {}; &
	\node[style=circuit-noop] (i-7) {}; &
	\node[style=circuit-ctrl] (i-X-a-4) {}; &
	\node[style=circuit-ctrl] (i-X-b-2) {}; &
	\node[style=circuit-gate] (i-X-i-1) {$X$}; &
	\node[style=circuit-ctrl] (i-X-b-3) {}; &
	\node[style=circuit-ctrl] (i-X-a-5) {}; \\

	\node[style=circuit-gate] (a-X-a-0) {$X$}; &
	\node[style=circuit-noop] (a-1) {}; &
	\node[style=circuit-noop] (a-2) {}; &
	\node[style=circuit-ctrl] (a-X-b-1) {}; &
	\node[style=circuit-gate] (a-X-a-1) {$X$}; &
	\node[style=circuit-gate] (a-X-a-2) {$X$}; &
	\node[style=circuit-ctrl] (a-X-r-0) {}; &
	\node[style=circuit-gate] (a-X-a-3) {$X$}; &
	\node[style=circuit-gate] (a-X-a-4) {$X$}; &
	\node[style=circuit-ctrl] (a-X-b-2) {}; &
	\node[style=circuit-noop] (a-10) {}; &
	\node[style=circuit-noop] (a-11) {}; &
	\node[style=circuit-gate] (a-X-a-5) {$X$}; \\

	\node[style=circuit-noop] (b-0) {}; &
	\node[style=circuit-gate] (b-X-b-0) {$X$}; &
	\node[style=circuit-noop] (b-2) {}; &
	\node[style=circuit-gate] (b-X-b-1) {$X$}; &
	\node[style=circuit-noop] (b-4) {}; &
	\node[style=circuit-ctrl] (b-X-a-2) {}; &
	\node[style=circuit-noop] (b-6) {}; &
	\node[style=circuit-ctrl] (b-X-a-3) {}; &
	\node[style=circuit-noop] (b-8) {}; &
	\node[style=circuit-gate] (b-X-b-2) {$X$}; &
	\node[style=circuit-noop] (b-10) {}; &
	\node[style=circuit-gate] (b-X-b-3) {$X$}; &
	\node[style=circuit-noop] (b-12) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-noop] (r-3) {}; &
	\node[style=circuit-noop] (r-4) {}; &
	\node[style=circuit-noop] (r-5) {}; &
	\node[style=circuit-gate] (r-X-r-0) {$X$}; &
	\node[style=circuit-noop] (r-7) {}; &
	\node[style=circuit-noop] (r-8) {}; &
	\node[style=circuit-noop] (r-9) {}; &
	\node[style=circuit-noop] (r-10) {}; &
	\node[style=circuit-noop] (r-11) {}; &
	\node[style=circuit-noop] (r-12) {}; \\
};
% COORDINATES
% i
\coordinate[left =\tikzWireLeft of i-X-a-0.center] (i-left);
\coordinate[right=\tikzWireRight of i-X-a-5.center] (i-right);

% a
\coordinate[left =\tikzWireLeft of a-X-a-0.center] (a-left);
\coordinate[right=\tikzWireRight of a-X-a-5.center] (a-right);

% b
\coordinate[left =\tikzWireLeft of b-0.center] (b-left);
\coordinate[right=\tikzWireRight of b-12.center] (b-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-12.center] (r-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (i-left) -- (i-right);
	\draw[-] (a-left) -- (a-right);
	\draw[-] (b-left) -- (b-right);
	\draw[-] (r-left) -- (r-right);

	% controls
	\draw[-] (i-X-a-0) -- (a-X-a-0);
	\draw[-] (i-X-b-0) -- (b-X-b-0);
	\draw[-] (i-X-b-1) -- (b-X-b-1);
	\draw[-] (a-X-b-1) -- (b-X-b-1);
	\draw[-] (i-X-a-1) -- (a-X-a-1);
	\draw[-] (b-X-a-2) -- (a-X-a-2);
	\draw[-] (a-X-r-0) -- (r-X-r-0);
	\draw[-] (b-X-a-3) -- (a-X-a-3);
	\draw[-] (i-X-a-4) -- (a-X-a-4);
	\draw[-] (i-X-b-2) -- (b-X-b-2);
	\draw[-] (a-X-b-2) -- (b-X-b-2);
	\draw[-] (i-X-b-3) -- (b-X-b-3);
	\draw[-] (i-X-a-5) -- (a-X-a-5);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(i-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$i$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(a-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_0$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(b-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_1$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};



==> figures/app_sq_incorrect_lazy.tex <==

\def\tikzRowSepDefault{2mm}
\def\tikzColumnSepDefault{0.9mm}
\def\tikzWireLeftDefault{0.7cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-ctrl] (i-X-a-0) {}; &
	\node[style=circuit-ctrl] (i-X-b-0) {}; &
	\node[style=circuit-gate] (i-X-i-0) {$X$}; &
	\node[style=circuit-ctrl] (i-X-b-1) {}; &
	\node[style=circuit-noop] (i-4) {}; &
	\node[style=circuit-noop] (i-5) {}; &
	\node[style=circuit-noop] (i-6) {}; &
	\node[style=circuit-ctrl] (i-X-b-2) {}; &
	\node[style=circuit-gate] (i-X-i-1) {$X$}; &
	\node[style=circuit-ctrl] (i-X-b-3) {}; &
	\node[style=circuit-ctrl] (i-X-a-1) {}; \\

	\node[style=circuit-gate] (a-X-a-0) {$X$}; &
	\node[style=circuit-noop] (a-1) {}; &
	\node[style=circuit-noop] (a-2) {}; &
	\node[style=circuit-ctrl] (a-X-b-1) {}; &
	\node[style=circuit-noop] (a-4) {}; &
	\node[style=circuit-noop] (a-5) {}; &
	\node[style=circuit-noop] (a-6) {}; &
	\node[style=circuit-ctrl] (a-X-b-2) {}; &
	\node[style=circuit-noop] (a-8) {}; &
	\node[style=circuit-noop] (a-9) {}; &
	\node[style=circuit-gate] (a-X-a-1) {$X$}; \\

	\node[style=circuit-noop] (b-0) {}; &
	\node[style=circuit-gate] (b-X-b-0) {$X$}; &
	\node[style=circuit-noop] (b-2) {}; &
	\node[style=circuit-gate] (b-X-b-1) {$X$}; &
	\node[style=circuit-ctrl] (b-X-c-0) {}; &
	\node[style=circuit-noop] (b-5) {}; &
	\node[style=circuit-ctrl] (b-X-c-1) {}; &
	\node[style=circuit-gate] (b-X-b-2) {$X$}; &
	\node[style=circuit-noop] (b-8) {}; &
	\node[style=circuit-gate] (b-X-b-3) {$X$}; &
	\node[style=circuit-noop] (b-10) {}; \\

	\node[style=circuit-noop] (c-0) {}; &
	\node[style=circuit-noop] (c-1) {}; &
	\node[style=circuit-noop] (c-2) {}; &
	\node[style=circuit-noop] (c-3) {}; &
	\node[style=circuit-gate] (c-X-c-0) {$X$}; &
	\node[style=circuit-ctrl] (c-X-r-0) {}; &
	\node[style=circuit-gate] (c-X-c-1) {$X$}; &
	\node[style=circuit-noop] (c-7) {}; &
	\node[style=circuit-noop] (c-8) {}; &
	\node[style=circuit-noop] (c-9) {}; &
	\node[style=circuit-noop] (c-10) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-noop] (r-3) {}; &
	\node[style=circuit-noop] (r-4) {}; &
	\node[style=circuit-gate] (r-X-r-0) {$X$}; &
	\node[style=circuit-noop] (r-6) {}; &
	\node[style=circuit-noop] (r-7) {}; &
	\node[style=circuit-noop] (r-8) {}; &
	\node[style=circuit-noop] (r-9) {}; &
	\node[style=circuit-noop] (r-10) {}; \\
};
% COORDINATES
% i
\coordinate[left =\tikzWireLeft of i-X-a-0.center] (i-left);
\coordinate[right=\tikzWireRight of i-X-a-1.center] (i-right);

% a
\coordinate[left =\tikzWireLeft of a-X-a-0.center] (a-left);
\coordinate[right=\tikzWireRight of a-X-a-1.center] (a-right);

% b
\coordinate[left =\tikzWireLeft of b-0.center] (b-left);
\coordinate[right=\tikzWireRight of b-10.center] (b-right);

% c
\coordinate[left =\tikzWireLeft of c-0.center] (c-left);
\coordinate[right=\tikzWireRight of c-10.center] (c-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-10.center] (r-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (i-left) -- (i-right);
	\draw[-] (a-left) -- (a-right);
	\draw[-] (b-left) -- (b-right);
	\draw[-] (c-left) -- (c-right);
	\draw[-] (r-left) -- (r-right);

	% controls
	\draw[-] (i-X-a-0) -- (a-X-a-0);
	\draw[-] (i-X-b-0) -- (b-X-b-0);
	\draw[-] (i-X-b-1) -- (b-X-b-1);
	\draw[-] (a-X-b-1) -- (b-X-b-1);
	\draw[-] (b-X-c-0) -- (c-X-c-0);
	\draw[-] (c-X-r-0) -- (r-X-r-0);
	\draw[-] (b-X-c-1) -- (c-X-c-1);
	\draw[-] (i-X-b-2) -- (b-X-b-2);
	\draw[-] (a-X-b-2) -- (b-X-b-2);
	\draw[-] (i-X-b-3) -- (b-X-b-3);
	\draw[-] (i-X-a-1) -- (a-X-a-1);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(i-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$i$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(a-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_0$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(b-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_1$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(c-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_2$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};



==> figures/circgraphuncomp/c6_0.tex <==
\scriptsize{
\begin{tikzpicture}
    %%%%%%%%%
    % NODES %
    %%%%%%%%%
    \matrix[row sep=\tikzMatrRowSep,column sep=\tikzMatrColSep] {
        \node (s00) [style=ttightgate, font=\scriptsize] {$s_{0.0}$}; &
        \node (a00) [style=ttightgate] {\scriptsize$a_{0.0}$}; &
        \node (b00) [style=ttightgate] {\scriptsize$t_{0.0}$};\\

        \node (s10) [style=ttightgate] {\scriptsize$s_{1.0}$}; & \node (a10) [style=ttightgate] {\scriptsize$a_{1.0}$}; &\\
        %&  & \\
        \node (s01) [style=ttightgate] {\scriptsize$s_{0.1}$}; & & \node (b10) [style=ttightgate] {\scriptsize$t_{1.0}$};\\
        %& & \\
         %& \node (a01) [style=ttightgate, fill=blue-node,text=blue-node-text] {\scriptsize$a_{0.1}$}; &\\
    };
    
    %\node (label) at (s00.west |- r10.east) {\scriptsize b) Circuit Graph $G$};

    %%%%%%%%%%%%%%%%
    % TARGET EDGES %
    %%%%%%%%%%%%%%%%


    \draw[style=targ] (s00) -- (s10);
    \draw[style=targ] (s10) -- (s01);

    \draw[style=targ] (a00) -- (a10);
    %\draw[style=targ] (a10) -- (a01);
    \draw[style=targ] (b00) -- (b10);

    %%%%%%%%%%%%%%%%%
    % CONTROL EDGES %
    %%%%%%%%%%%%%%%%%

    \draw[style=ctrl] (s10.east) -- (a10.west);
    \draw[style=ctrl] (a10) -- (b10);
    \draw[style=ctrl] (s01.east) -- (b10.west);

    %%%%%%%%%%%%%%%%%
    % AVAIL EDGES %
    %%%%%%%%%%%%%%%%%

    \draw[style=avail] (a10) -- (s01);
    %\draw[style=avail] (b10) -- (a01);

 \end{tikzpicture}
}




==> figures/circgraphuncomp/c6_1.tex <==
\scriptsize{
\begin{tikzpicture}
    %%%%%%%%%
    % NODES %
    %%%%%%%%%
    \matrix[row sep=\tikzMatrRowSep,column sep=\tikzMatrColSep] {
        \node (s00) [style=ttightgate, font=\scriptsize] {$s_{0.0}$}; &
        \node (a00) [style=ttightgate] {\scriptsize$a_{0.0}$}; &
        \node (b00) [style=ttightgate] {\scriptsize$t_{0.0}$};\\

        \node (s10) [style=ttightgate] {\scriptsize$s_{1.0}$}; & \node (a10) [style=ttightgate] {\scriptsize$a_{1.0}$}; &\\
        %&  & \\
        \node (s01) [style=ttightgate] {\scriptsize$s_{0.1}$}; & & \node (b10) [style=ttightgate] {\scriptsize$t_{1.0}$};\\
        
        %& & \\
         & \node (a01) [style=ttightgate, fill=blue-node,text=blue-node-text] {\scriptsize$a_{0.1}$}; &\\
    };
    
    %\node (label) at (s00.west |- r10.east) {\scriptsize b) Circuit Graph $G$};

    %%%%%%%%%%%%%%%%
    % TARGET EDGES %
    %%%%%%%%%%%%%%%%


    \draw[style=targ] (s00) -- (s10);
    \draw[style=targ] (s10) -- (s01);

    \draw[style=targ] (a00) -- (a10);
    \draw[style=targ] (a10) -- (a01);
    \draw[style=targ] (b00) -- (b10);

    %%%%%%%%%%%%%%%%%
    % CONTROL EDGES %
    %%%%%%%%%%%%%%%%%

    \draw[style=ctrl] (s10.east) -- (a10.west);
    \draw[style=ctrl] (a10) -- (b10);
    \draw[style=ctrl] (s01.east) -- (b10.west);
    \node (mida01) at ($(a01.north west)!0.1!(a01.north east)$) {};
    \draw[style=ctrl,color=red-node] (s10) edge[bend left=15] node {} (mida01);

    %%%%%%%%%%%%%%%%%
    % AVAIL EDGES %
    %%%%%%%%%%%%%%%%%

    \draw[style=avail] (a10) -- (s01);
    \draw[style=avail] (b10) -- (a01);
    \draw[style=avail,color=red-node] (a01) -- (s01);

 \end{tikzpicture}
}




==> figures/circgraphuncomp/c6_2.tex <==
\scriptsize{
\begin{tikzpicture}
    %%%%%%%%%
    % NODES %
    %%%%%%%%%
    \matrix[row sep=\tikzMatrRowSep,column sep=\tikzMatrColSep] {
        \node (s00) [style=ttightgate, font=\scriptsize] {$s_{0.0}$}; &
        \node (a00) [style=ttightgate] {\scriptsize$a_{0.0}$}; &
        \node (b00) [style=ttightgate] {\scriptsize$t_{0.0}$};\\

        \node (s10) [style=ttightgate] {\scriptsize$s_{1.0}$}; & \node (a10) [style=ttightgate] {\scriptsize$a_{1.0}$}; &\\
        %&  & \\
        \node (s01) [style=ttightgate] {\scriptsize$s_{0.1}$}; & & \node (b10) [style=ttightgate] {\scriptsize$t_{1.0}$};\\
        
        %& & \\
        \node (s11) [style=ttightgate, fill=green-node,text=green-node-text] {\scriptsize$s_{1.1}$}; & \node (a01) [style=ttightgate, fill=blue-node,text=blue-node-text] {\scriptsize$a_{0.1}$}; &\\
    };
    
    %\node (label) at (s00.west |- r10.east) {\scriptsize b) Circuit Graph $G$};

    %%%%%%%%%%%%%%%%
    % TARGET EDGES %
    %%%%%%%%%%%%%%%%


    \draw[style=targ] (s00) -- (s10);
    \draw[style=targ] (s10) -- (s01);
    \draw[style=targ] (s01) -- (s11);

    \draw[style=targ] (a00) -- (a10);
    \draw[style=targ] (a10) -- (a01);
    \draw[style=targ] (b00) -- (b10);

    %%%%%%%%%%%%%%%%%
    % CONTROL EDGES %
    %%%%%%%%%%%%%%%%%

    \draw[style=ctrl] (s10.east) -- (a10.west);
    \draw[style=ctrl] (s11.east) -- (a01.west);
    \draw[style=ctrl] (a10) -- (b10);
    \draw[style=ctrl] (s01.east) -- (b10.west);

    %%%%%%%%%%%%%%%%%
    % AVAIL EDGES %
    %%%%%%%%%%%%%%%%%

    \draw[style=avail] (a10) -- (s01);
    \draw[style=avail] (b10) -- (s11.north east);
    \draw[style=avail] (b10) -- (a01);

 \end{tikzpicture}
}




==> figures/eval_unqomp_cannot.tex <==


\def\tikzRowSepDefault{2mm}
\def\tikzColumnSepDefault{0.5mm}
\def\tikzWireLeftDefault{1cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-gate] (p-X-p-0) {$X$}; &
	\node[style=circuit-ctrl] (p-X-a-0) {}; &
	\node[style=circuit-gate] (p-X-p-1) {$X$}; &
	\node[style=circuit-noop] (p-3) {}; &
	\node[style=circuit-ctrl] (p-X-r-0) {}; &
	\node[style=circuit-noop] (p-5) {}; &
	\node[style=circuit-gate] (p-X-p-2) {$X$}; &
	\node[style=circuit-ctrl] (p-X-a-1) {}; &
	\node[style=circuit-gate] (p-X-p-3) {$X$}; \\

	\node[style=circuit-noop] (a-0) {}; &
	\node[style=circuit-gate] (a-X-a-0) {$X$}; &
	\node[style=circuit-noop] (a-2) {}; &
	\node[style=circuit-noop] (a-3) {}; &
	\node[style=circuit-ctrl] (a-X-r-0) {}; &
	\node[style=circuit-noop] (a-5) {}; &
	\node[style=circuit-noop] (a-6) {}; &
	\node[style=circuit-gate] (a-X-a-1) {$X$}; &
	\node[style=circuit-noop] (a-8) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-noop] (r-3) {}; &
	\node[style=circuit-gate] (r-X-r-0) {$X$}; &
	\node[style=circuit-noop] (r-5) {}; &
	\node[style=circuit-noop] (r-6) {}; &
	\node[style=circuit-noop] (r-7) {}; &
	\node[style=circuit-noop] (r-8) {}; \\
};
% COORDINATES
% p
\coordinate[left =\tikzWireLeft of p-X-p-0.center] (p-left);
\coordinate[right=\tikzWireRight of p-X-p-3.center] (p-right);

% a
\coordinate[left =\tikzWireLeft of a-0.center] (a-left);
\coordinate[right=\tikzWireRight of a-8.center] (a-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-8.center] (r-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (p-left) -- (p-right);
	\draw[-] (a-left) -- (a-right);
	\draw[-] (r-left) -- (r-right);

	% controls
	\draw[-] (p-X-a-0) -- (a-X-a-0);
	\draw[-] (p-X-r-0) -- (r-X-r-0);
	\draw[-] (a-X-r-0) -- (r-X-r-0);
	\draw[-] (p-X-a-1) -- (a-X-a-1);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] (p-label) at ($(p-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$p$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(a-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$a$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};



==> figures/pb_stmt_circ.tex <==
\def\tikzRowSepDefault{1mm}
\def\tikzColumnSepDefault{0.5mm}
\def\tikzWireLeftDefault{1cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-ctrl] (o-X-v0-0) {}; &
	\node[style=circuit-noop] (o-1) {}; &
	\node[style=circuit-noop] (o-2) {}; &
	\node[style=circuit-noop] (o-3) {}; \\

	\node[style=circuit-ctrl] (p-X-v0-0) {}; &
	\node[style=circuit-noop] (p-1) {}; &
	\node[style=circuit-noop] (p-2) {}; &
	\node[style=circuit-noop] (p-3) {}; \\

	\node[style=circuit-noop] (q-0) {}; &
	\node[style=circuit-ctrl] (q-X-v1-0) {}; &
	\node[style=circuit-noop] (q-2) {}; &
	\node[style=circuit-noop] (q-3) {}; \\

	\node[style=circuit-noop] (s-0) {}; &
	\node[style=circuit-noop] (s-1) {}; &
	\node[style=circuit-ctrl] (s-X-v2-0) {}; &
	\node[style=circuit-noop] (s-3) {}; \\

	\node[style=circuit-gate] (v0-X-v0-0) {$X$}; &
	\node[style=circuit-ctrl] (v0-X-v1-0) {}; &
	\node[style=circuit-noop] (v0-2) {}; &
	\node[style=circuit-noop] (v0-3) {}; \\

	\node[style=circuit-noop] (v1-0) {}; &
	\node[style=circuit-gate] (v1-X-v1-0) {$X$}; &
	\node[style=circuit-ctrl] (v1-X-v2-0) {}; &
	\node[style=circuit-noop] (v1-3) {}; \\

	\node[style=circuit-noop] (v2-0) {}; &
	\node[style=circuit-noop] (v2-1) {}; &
	\node[style=circuit-gate] (v2-X-v2-0) {$X$}; &
	\node[style=circuit-ctrl] (v2-H-r-0) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-gate] (r-H-r-0) {$H$}; \\
};
% COORDINATES
% o
\coordinate[left =\tikzWireLeft of o-X-v0-0.center] (o-left);
\coordinate[right=\tikzWireRight of o-3.center] (o-right);

% p
\coordinate[left =\tikzWireLeft of p-X-v0-0.center] (p-left);
\coordinate[right=\tikzWireRight of p-3.center] (p-right);

% q
\coordinate[left =\tikzWireLeft of q-0.center] (q-left);
\coordinate[right=\tikzWireRight of q-3.center] (q-right);

% s
\coordinate[left =\tikzWireLeft of s-0.center] (s-left);
\coordinate[right=\tikzWireRight of s-3.center] (s-right);

% v0
\coordinate[left =\tikzWireLeft of v0-X-v0-0.center] (v0-left);
\coordinate[right=\tikzWireRight of v0-3.center] (v0-right);

% v1
\coordinate[left =\tikzWireLeft of v1-0.center] (v1-left);
\coordinate[right=\tikzWireRight of v1-3.center] (v1-right);

% v2
\coordinate[left =\tikzWireLeft of v2-0.center] (v2-left);
\coordinate[right=\tikzWireRight of v2-H-r-0.center] (v2-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-H-r-0.center] (r-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (o-left) -- (o-right);
	\draw[-] (p-left) -- (p-right);
	\draw[-] (q-left) -- (q-right);
	\draw[-] (s-left) -- (s-right);
	\draw[-] (v0-left) -- (v0-right);
	\draw[-] (v1-left) -- (v1-right);
	\draw[-] (v2-left) -- (v2-right);
	\draw[-] (r-left) -- (r-right);

	% controls
	\draw[-] (o-X-v0-0) -- (v0-X-v0-0);
	\draw[-] (p-X-v0-0) -- (v0-X-v0-0);
	\draw[-] (q-X-v1-0) -- (v1-X-v1-0);
	\draw[-] (v0-X-v1-0) -- (v1-X-v1-0);
	\draw[-] (s-X-v2-0) -- (v2-X-v2-0);
	\draw[-] (v1-X-v2-0) -- (v2-X-v2-0);
	\draw[-] (v2-H-r-0) -- (r-H-r-0);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(o-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$o$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(p-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$p$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(q-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$q$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(s-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v0-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_0$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v1-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_1$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v2-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_2$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$t$};



==> figures/pb_stmt_eager_circ.tex <==

\def\tikzRowSepDefault{1mm}
\def\tikzColumnSepDefault{0.5mm}
\def\tikzWireLeftDefault{1cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-ctrl] (o-X-v0-0) {}; &
	\node[style=circuit-noop] (o-1) {}; &
	\node[style=circuit-ctrl] (o-X-v0-1) {}; &
	\node[style=circuit-noop] (o-3) {}; &
	\node[style=circuit-noop] (o-4) {}; &
	\node[style=circuit-noop] (o-5) {}; &
	\node[style=circuit-noop] (o-6) {}; &
	\node[style=circuit-noop] (o-7) {}; &
	\node[style=circuit-ctrl] (o-X-v0-4) {}; &
	\node[style=circuit-noop] (o-9) {}; &
	\node[style=circuit-ctrl] (o-X-v0-5) {}; \\

	\node[style=circuit-ctrl] (p-X-v0-0) {}; &
	\node[style=circuit-noop] (p-1) {}; &
	\node[style=circuit-ctrl] (p-X-v0-1) {}; &
	\node[style=circuit-noop] (p-3) {}; &
	\node[style=circuit-noop] (p-4) {}; &
	\node[style=circuit-noop] (p-5) {}; &
	\node[style=circuit-noop] (p-6) {}; &
	\node[style=circuit-noop] (p-7) {}; &
	\node[style=circuit-ctrl] (p-X-v0-4) {}; &
	\node[style=circuit-noop] (p-9) {}; &
	\node[style=circuit-ctrl] (p-X-v0-5) {}; \\

	\node[style=circuit-noop] (q-0) {}; &
	\node[style=circuit-ctrl] (q-X-v1-0) {}; &
	\node[style=circuit-noop] (q-2) {}; &
	\node[style=circuit-noop] (q-3) {}; &
	\node[style=circuit-noop] (q-4) {}; &
	\node[style=circuit-noop] (q-5) {}; &
	\node[style=circuit-noop] (q-6) {}; &
	\node[style=circuit-noop] (q-7) {}; &
	\node[style=circuit-noop] (q-8) {}; &
	\node[style=circuit-ctrl] (q-X-v1-1) {}; &
	\node[style=circuit-noop] (q-10) {}; \\

	\node[style=circuit-noop] (s-0) {}; &
	\node[style=circuit-noop] (s-1) {}; &
	\node[style=circuit-noop] (s-2) {}; &
	\node[style=circuit-noop] (s-3) {}; &
	\node[style=circuit-ctrl] (s-X-v0-2) {}; &
	\node[style=circuit-noop] (s-5) {}; &
	\node[style=circuit-ctrl] (s-X-v0-3) {}; &
	\node[style=circuit-noop] (s-7) {}; &
	\node[style=circuit-noop] (s-8) {}; &
	\node[style=circuit-noop] (s-9) {}; &
	\node[style=circuit-noop] (s-10) {}; \\

	\node[style=circuit-gate] (v0-X-v0-0) {$X$}; &
	\node[style=circuit-ctrl] (v0-X-v1-0) {}; &
	\node[style=circuit-gate] (v0-X-v0-1) {$X$}; &
	\node[style=circuit-noop] (v0-3) {}; &
	\node[style=circuit-gate] (v0-X-v0-2) {$X$}; &
	\node[style=circuit-ctrl] (v0-H-r-0) {}; &
	\node[style=circuit-gate] (v0-X-v0-3) {$X$}; &
	\node[style=circuit-noop] (v0-7) {}; &
	\node[style=circuit-gate] (v0-X-v0-4) {$X$}; &
	\node[style=circuit-ctrl] (v0-X-v1-1) {}; &
	\node[style=circuit-gate] (v0-X-v0-5) {$X$}; \\

	\node[style=circuit-noop] (v1-0) {}; &
	\node[style=circuit-gate] (v1-X-v1-0) {$X$}; &
	\node[style=circuit-noop] (v1-2) {}; &
	\node[style=circuit-noop] (v1-3) {}; &
	\node[style=circuit-ctrl] (v1-X-v0-2) {}; &
	\node[style=circuit-noop] (v1-5) {}; &
	\node[style=circuit-ctrl] (v1-X-v0-3) {}; &
	\node[style=circuit-noop] (v1-7) {}; &
	\node[style=circuit-noop] (v1-8) {}; &
	\node[style=circuit-gate] (v1-X-v1-1) {$X$}; &
	\node[style=circuit-noop] (v1-10) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-noop] (r-3) {}; &
	\node[style=circuit-noop] (r-4) {}; &
	\node[style=circuit-gate] (r-H-r-0) {$H$}; &
	\node[style=circuit-noop] (r-6) {}; &
	\node[style=circuit-noop] (r-7) {}; &
	\node[style=circuit-noop] (r-8) {}; &
	\node[style=circuit-noop] (r-9) {}; &
	\node[style=circuit-noop] (r-10) {}; \\
};
% COORDINATES
% o
\coordinate[left =\tikzWireLeft of o-X-v0-0.center] (o-left);
\coordinate[right=\tikzWireRight of o-X-v0-5.center] (o-right);

% p
\coordinate[left =\tikzWireLeft of p-X-v0-0.center] (p-left);
\coordinate[right=\tikzWireRight of p-X-v0-5.center] (p-right);

% q
\coordinate[left =\tikzWireLeft of q-0.center] (q-left);
\coordinate[right=\tikzWireRight of q-10.center] (q-right);

% s
\coordinate[left =\tikzWireLeft of s-0.center] (s-left);
\coordinate[right=\tikzWireRight of s-10.center] (s-right);

% v0
\coordinate[left =\tikzWireLeft of v0-X-v0-0.center] (v0-left);
\coordinate[right=\tikzWireRight of v0-X-v0-5.center] (v0-right);

% v1
\coordinate[left =\tikzWireLeft of v1-0.center] (v1-left);
\coordinate[right=\tikzWireRight of v1-10.center] (v1-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-10.center] (r-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (o-left) -- (o-right);
	\draw[-] (p-left) -- (p-right);
	\draw[-] (q-left) -- (q-right);
	\draw[-] (s-left) -- (s-right);
	\draw[-] (v0-left) -- (v0-right);
	\draw[-] (v1-left) -- (v1-right);
	\draw[-] (r-left) -- (r-right);

	% controls
	\draw[-] (o-X-v0-0) -- (v0-X-v0-0);
	\draw[-] (p-X-v0-0) -- (v0-X-v0-0);
	\draw[-] (q-X-v1-0) -- (v1-X-v1-0);
	\draw[-] (v0-X-v1-0) -- (v1-X-v1-0);
	\draw[-] (o-X-v0-1) -- (v0-X-v0-1);
	\draw[-] (p-X-v0-1) -- (v0-X-v0-1);
	\draw[-] (s-X-v0-2) -- (v0-X-v0-2);
	\draw[-] (v1-X-v0-2) -- (v0-X-v0-2);
	\draw[-] (v0-H-r-0) -- (r-H-r-0);
	\draw[-] (s-X-v0-3) -- (v0-X-v0-3);
	\draw[-] (v1-X-v0-3) -- (v0-X-v0-3);
	\draw[-] (o-X-v0-4) -- (v0-X-v0-4);
	\draw[-] (p-X-v0-4) -- (v0-X-v0-4);
	\draw[-] (q-X-v1-1) -- (v1-X-v1-1);
	\draw[-] (v0-X-v1-1) -- (v1-X-v1-1);
	\draw[-] (o-X-v0-5) -- (v0-X-v0-5);
	\draw[-] (p-X-v0-5) -- (v0-X-v0-5);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(o-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$o$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(p-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$p$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(q-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$q$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(s-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v0-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_0$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v1-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_1$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$t$};



==> figures/pb_stmt_lazy_circ.tex <==

\def\tikzRowSepDefault{1mm}
\def\tikzColumnSepDefault{0.5mm}
\def\tikzWireLeftDefault{1cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-ctrl] (o-X-v0-0) {}; &
	\node[style=circuit-noop] (o-1) {}; &
	\node[style=circuit-noop] (o-2) {}; &
	\node[style=circuit-noop] (o-3) {}; &
	\node[style=circuit-noop] (o-4) {}; &
	\node[style=circuit-noop] (o-5) {}; &
	\node[style=circuit-ctrl] (o-X-v0-1) {}; \\

	\node[style=circuit-ctrl] (p-X-v0-0) {}; &
	\node[style=circuit-noop] (p-1) {}; &
	\node[style=circuit-noop] (p-2) {}; &
	\node[style=circuit-noop] (p-3) {}; &
	\node[style=circuit-noop] (p-4) {}; &
	\node[style=circuit-noop] (p-5) {}; &
	\node[style=circuit-ctrl] (p-X-v0-1) {}; \\

	\node[style=circuit-noop] (q-0) {}; &
	\node[style=circuit-ctrl] (q-X-v1-0) {}; &
	\node[style=circuit-noop] (q-2) {}; &
	\node[style=circuit-noop] (q-3) {}; &
	\node[style=circuit-noop] (q-4) {}; &
	\node[style=circuit-ctrl] (q-X-v1-1) {}; &
	\node[style=circuit-noop] (q-6) {}; \\

	\node[style=circuit-noop] (s-0) {}; &
	\node[style=circuit-noop] (s-1) {}; &
	\node[style=circuit-ctrl] (s-X-v2-0) {}; &
	\node[style=circuit-noop] (s-3) {}; &
	\node[style=circuit-ctrl] (s-X-v2-1) {}; &
	\node[style=circuit-noop] (s-5) {}; &
	\node[style=circuit-noop] (s-6) {}; \\

	\node[style=circuit-gate] (v0-X-v0-0) {$X$}; &
	\node[style=circuit-ctrl] (v0-X-v1-0) {}; &
	\node[style=circuit-noop] (v0-2) {}; &
	\node[style=circuit-noop] (v0-3) {}; &
	\node[style=circuit-noop] (v0-4) {}; &
	\node[style=circuit-ctrl] (v0-X-v1-1) {}; &
	\node[style=circuit-gate] (v0-X-v0-1) {$X$}; \\

	\node[style=circuit-noop] (v1-0) {}; &
	\node[style=circuit-gate] (v1-X-v1-0) {$X$}; &
	\node[style=circuit-ctrl] (v1-X-v2-0) {}; &
	\node[style=circuit-noop] (v1-3) {}; &
	\node[style=circuit-ctrl] (v1-X-v2-1) {}; &
	\node[style=circuit-gate] (v1-X-v1-1) {$X$}; &
	\node[style=circuit-noop] (v1-6) {}; \\

	\node[style=circuit-noop] (v2-0) {}; &
	\node[style=circuit-noop] (v2-1) {}; &
	\node[style=circuit-gate] (v2-X-v2-0) {$X$}; &
	\node[style=circuit-ctrl] (v2-H-r-0) {}; &
	\node[style=circuit-gate] (v2-X-v2-1) {$X$}; &
	\node[style=circuit-noop] (v2-5) {}; &
	\node[style=circuit-noop] (v2-6) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-gate] (r-H-r-0) {$H$}; &
	\node[style=circuit-noop] (r-4) {}; &
	\node[style=circuit-noop] (r-5) {}; &
	\node[style=circuit-noop] (r-6) {}; \\
};
% COORDINATES
% o
\coordinate[left =\tikzWireLeft of o-X-v0-0.center] (o-left);
\coordinate[right=\tikzWireRight of o-X-v0-1.center] (o-right);

% p
\coordinate[left =\tikzWireLeft of p-X-v0-0.center] (p-left);
\coordinate[right=\tikzWireRight of p-X-v0-1.center] (p-right);

% q
\coordinate[left =\tikzWireLeft of q-0.center] (q-left);
\coordinate[right=\tikzWireRight of q-6.center] (q-right);

% s
\coordinate[left =\tikzWireLeft of s-0.center] (s-left);
\coordinate[right=\tikzWireRight of s-6.center] (s-right);

% v0
\coordinate[left =\tikzWireLeft of v0-X-v0-0.center] (v0-left);
\coordinate[right=\tikzWireRight of v0-X-v0-1.center] (v0-right);

% v1
\coordinate[left =\tikzWireLeft of v1-0.center] (v1-left);
\coordinate[right=\tikzWireRight of v1-6.center] (v1-right);

% v2
\coordinate[left =\tikzWireLeft of v2-0.center] (v2-left);
\coordinate[right=\tikzWireRight of v2-6.center] (v2-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-6.center] (r-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (o-left) -- (o-right);
	\draw[-] (p-left) -- (p-right);
	\draw[-] (q-left) -- (q-right);
	\draw[-] (s-left) -- (s-right);
	\draw[-] (v0-left) -- (v0-right);
	\draw[-] (v1-left) -- (v1-right);
	\draw[-] (v2-left) -- (v2-right);
	\draw[-] (r-left) -- (r-right);

	% controls
	\draw[-] (o-X-v0-0) -- (v0-X-v0-0);
	\draw[-] (p-X-v0-0) -- (v0-X-v0-0);
	\draw[-] (q-X-v1-0) -- (v1-X-v1-0);
	\draw[-] (v0-X-v1-0) -- (v1-X-v1-0);
	\draw[-] (s-X-v2-0) -- (v2-X-v2-0);
	\draw[-] (v1-X-v2-0) -- (v2-X-v2-0);
	\draw[-] (v2-H-r-0) -- (r-H-r-0);
	\draw[-] (s-X-v2-1) -- (v2-X-v2-1);
	\draw[-] (v1-X-v2-1) -- (v2-X-v2-1);
	\draw[-] (q-X-v1-1) -- (v1-X-v1-1);
	\draw[-] (v0-X-v1-1) -- (v1-X-v1-1);
	\draw[-] (o-X-v0-1) -- (v0-X-v0-1);
	\draw[-] (p-X-v0-1) -- (v0-X-v0-1);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(o-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$o$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(p-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$p$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(q-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$q$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(s-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v0-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_0$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v1-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_1$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v2-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u_2$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$t$};



==> figures/reqomp-fig/circgraph.tex <==
\scriptsize{
\begin{tikzpicture}
    %%%%%%%%%
    % NODES %
    %%%%%%%%%
    \matrix[row sep=3mm,column sep=9mm] {
        \node (a00) [style=ttightgate] {\scriptsize$a_{0.0}$}; &
        \node (b00) [style=ttightgate] {\scriptsize$b_{0.0}$}; &
        \node (c00) [style=ttightgate] {\scriptsize$c_{0.0}$}; &
        \node (r00) [style=ttightgate] {\scriptsize$r_{0.0}$}; &
        \node (d00) [style=ttightgate] {\scriptsize$d_{0.0}$}; &
        \node (e00) [style=ttightgate] {\scriptsize$e_{0.0}$};&
        \node (t00) [style=ttightgate] {\scriptsize$t_{0.0}$}; \\

        \node (a10) [style=ttightgate] {\scriptsize$a_{1.0}$}; &
        \node (b10) [style=ttightgate] {\scriptsize$b_{1.0}$}; &
         & & & \\

        & &
        \node (c10) [style=ttightgate] {\scriptsize$c_{1.0}$}; & \\

        & & & \node (r10) [style=ttightgate] {\scriptsize$r_{1.0}$}; &
        \node (d10) [style=ttightgate] {\scriptsize$d_{1.0}$}; &
        \node (e10) [style=ttightgate] {\scriptsize$e_{1.0}$}; \\

        & & & & & &
        \node (t10) [style=ttightgate] {\scriptsize$t_{2.0}$};\\
    };

    \node (a10l) at (a10.south) [anchor=south, style=ttightgate] {\scriptsize$a_{1.0} : X$};
    \node (b10l) at (b10.south) [anchor=south, style=ttightgate] {\scriptsize$b_{1.0} : CX$};

    \node (c10l) at (c10.south) [anchor=south, style=ttightgate] {\scriptsize$c_{1.0} : CCX$};
    \node (r10l) at (r10.south) [anchor=south, style=ttightgate] {\scriptsize$r_{1.0} : CH$};
    \node (d10l) at (d10.south) [anchor=south, style=ttightgate] {\scriptsize$d_{1.0} : CX$};
    \node (e10l) at (e10.south) [anchor=south, style=ttightgate] {\scriptsize$e_{1.0} : CX$};

    \node (t10l) at (t10.south) [anchor=south, style=ttightgate] {\scriptsize$t_{1.0} : CH$};
    %\node (label) at (s00.west |- r10.east) {\scriptsize b) Circuit Graph $G$};

    %%%%%%%%%%%%%%%%
    % TARGET EDGES %
    %%%%%%%%%%%%%%%%


    \draw[style=targ] (a00) -- (a10);
    \draw[style=targ] (b00) -- (b10);
    \draw[style=targ] (c00) -- (c10);
    \draw[style=targ] (d00) -- (d10);
    \draw[style=targ] (e00) -- (e10);
    \draw[style=targ] (r00) -- (r10);
    \draw[style=targ] (t00) -- (t10);

    %%%%%%%%%%%%%%%%%
    % CONTROL EDGES %
    %%%%%%%%%%%%%%%%%

    \draw[style=ctrl] (a10l.east) -- (b10l.west);
    \draw[style=ctrl] (b10l) -- (c10l);
    \draw[style=ctrl] (c10l) -- (r10l);
    \draw[style=ctrl] (r10l) -- (d10l);
    \draw[style=ctrl] (d10l) -- (e10l);
    \draw[style=ctrl] (e10l) -- (t10l);

    %%%%%%%%%%%%%%%%%
    % AVAIL EDGES %
    %%%%%%%%%%%%%%%%%

    %\draw[style=avail] (a10) -- (s01);

    \begin{scope}[on background layer]
        \draw [split=0.1cm, color= my-full-red!40]
            (a00.north west) -- % top left
           (a00.north east) -- % top left
           (a00.south east) -- % top left
           (a00.south) -- % top left
            (a10l.north) -- % top right
           (a10l.north east) -- % top right
            (a10l.south east) -- % bottom right
            (a10l.south west) -- % bottom left
           (a10l.north west) -- % bottom left
           (a10l.north) -- % bottom left
           (a00.south) -- % bottom left
           (a00.south west) -- % bottom left
            cycle;

    \draw [split=0.1cm, color= my-full-red!40]
            (b00.north west) -- % top left
           (b00.north east) -- % top left
           (b00.south east) -- % top left
           (b00.south) -- % top left
            (b10l.north) -- % top right
           (b10l.north east) -- % top right
            (b10l.south east) -- % bottom right
            (b10l.south west) -- % bottom left
           (b10l.north west) -- % bottom left
           (b10l.north) -- % bottom left
           (b00.south) -- % bottom left
           (b00.south west) -- % bottom left
            cycle;

       \draw [split=0.1cm, color= my-full-red!40]
            (c00.north west) -- % top left
           (c00.north east) -- % top left
           (c00.south east) -- % top left
           (c00.south) -- % top left
            (c10l.north) -- % top right
           (c10l.north east) -- % top right
            (c10l.south east) -- % bottom right
            (c10l.south west) -- % bottom left
           (c10l.north west) -- % bottom left
           (c10l.north) -- % bottom left
           (c00.south) -- % bottom left
           (c00.south west) -- % bottom left
            cycle;

        \draw [split=0.1cm, color= my-full-red!40]
            (d00.north west) -- % top left
           (d00.north east) -- % top left
           (d00.south east) -- % top left
           (d00.south) -- % top left
            (d10l.north) -- % top right
           (d10l.north east) -- % top right
            (d10l.south east) -- % bottom right
            (d10l.south west) -- % bottom left
           (d10l.north west) -- % bottom left
           (d10l.north) -- % bottom left
           (d00.south) -- % bottom left
           (d00.south west) -- % bottom left
            cycle;

        \draw [split=0.1cm, color= my-full-red!40]
            (e00.north west) -- % top left
           (e00.north east) -- % top left
           (e00.south east) -- % top left
           (e00.south) -- % top left
            (e10l.north) -- % top right
           (e10l.north east) -- % top right
            (e10l.south east) -- % bottom right
            (e10l.south west) -- % bottom left
           (e10l.north west) -- % bottom left
           (e10l.north) -- % bottom left
           (e00.south) -- % bottom left
           (e00.south west) -- % bottom left
            cycle;


       \draw[-,line width=0.2cm, color = my-full-blue!60] (a10) -- (b10);
       \draw[-,line width=0.2cm, color = my-full-blue!60] (b10) -- (c10);
       \draw[-,line width=0.2cm, color = my-full-blue!60] (d10) -- (e10);
    \end{scope}

 \end{tikzpicture}
}




==> figures/reqomp-fig/circuit.tex <==

\def\tikzRowSepDefault{2mm}
\def\tikzColumnSepDefault{0.5mm}
\def\tikzWireLeftDefault{1cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-gate] (a-X-a-0) {$X$}; &
	\node[style=circuit-ctrl] (a-X-b-0) {}; &
	\node[style=circuit-noop] (a-2) {}; &
	\node[style=circuit-noop] (a-3) {}; &
	\node[style=circuit-noop] (a-4) {}; &
	\node[style=circuit-noop] (a-5) {}; &
	\node[style=circuit-noop] (a-6) {}; \\

	\node[style=circuit-noop] (b-0) {}; &
	\node[style=circuit-gate] (b-X-b-0) {$X$}; &
	\node[style=circuit-ctrl] (b-X-c-0) {}; &
	\node[style=circuit-noop] (b-3) {}; &
	\node[style=circuit-noop] (b-4) {}; &
	\node[style=circuit-noop] (b-5) {}; &
	\node[style=circuit-noop] (b-6) {}; \\

	\node[style=circuit-noop] (c-0) {}; &
	\node[style=circuit-noop] (c-1) {}; &
	\node[style=circuit-gate] (c-X-c-0) {$X$}; &
	\node[style=circuit-ctrl] (c-H-r-0) {}; &
	\node[style=circuit-noop] (c-4) {}; &
	\node[style=circuit-noop] (c-5) {}; &
	\node[style=circuit-noop] (c-6) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-gate] (r-H-r-0) {$H$}; &
	\node[style=circuit-ctrl] (r-X-d-0) {}; &
	\node[style=circuit-noop] (r-5) {}; &
	\node[style=circuit-noop] (r-6) {}; \\

	\node[style=circuit-noop] (d-0) {}; &
	\node[style=circuit-noop] (d-1) {}; &
	\node[style=circuit-noop] (d-2) {}; &
	\node[style=circuit-noop] (d-3) {}; &
	\node[style=circuit-gate] (d-X-d-0) {$X$}; &
	\node[style=circuit-ctrl] (d-X-e-0) {}; &
	\node[style=circuit-noop] (d-6) {}; \\

	\node[style=circuit-noop] (e-0) {}; &
	\node[style=circuit-noop] (e-1) {}; &
	\node[style=circuit-noop] (e-2) {}; &
	\node[style=circuit-noop] (e-3) {}; &
	\node[style=circuit-noop] (e-4) {}; &
	\node[style=circuit-gate] (e-X-e-0) {$X$}; &
	\node[style=circuit-ctrl] (e-H-t-0) {}; \\

	\node[style=circuit-noop] (t-0) {}; &
	\node[style=circuit-noop] (t-1) {}; &
	\node[style=circuit-noop] (t-2) {}; &
	\node[style=circuit-noop] (t-3) {}; &
	\node[style=circuit-noop] (t-4) {}; &
	\node[style=circuit-noop] (t-5) {}; &
	\node[style=circuit-gate] (t-H-t-0) {$H$}; \\
};
% COORDINATES
% a
\coordinate[left =\tikzWireLeft of a-X-a-0.center] (a-left);
\coordinate[right=\tikzWireRight of a-6.center] (a-right);

% b
\coordinate[left =\tikzWireLeft of b-0.center] (b-left);
\coordinate[right=\tikzWireRight of b-6.center] (b-right);

% c
\coordinate[left =\tikzWireLeft of c-0.center] (c-left);
\coordinate[right=\tikzWireRight of c-6.center] (c-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-6.center] (r-right);

% d
\coordinate[left =\tikzWireLeft of d-0.center] (d-left);
\coordinate[right=\tikzWireRight of d-6.center] (d-right);

% e
\coordinate[left =\tikzWireLeft of e-0.center] (e-left);
\coordinate[right=\tikzWireRight of e-H-t-0.center] (e-right);

% t
\coordinate[left =\tikzWireLeft of t-0.center] (t-left);
\coordinate[right=\tikzWireRight of t-H-t-0.center] (t-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (a-left) -- (a-right);
	\draw[-] (b-left) -- (b-right);
	\draw[-] (c-left) -- (c-right);
	\draw[-] (r-left) -- (r-right);
	\draw[-] (d-left) -- (d-right);
	\draw[-] (e-left) -- (e-right);
	\draw[-] (t-left) -- (t-right);

	% controls
	\draw[-] (a-X-b-0) -- (b-X-b-0);
	\draw[-] (b-X-c-0) -- (c-X-c-0);
	\draw[-] (c-H-r-0) -- (r-H-r-0);
	\draw[-] (r-X-d-0) -- (d-X-d-0);
	\draw[-] (d-X-e-0) -- (e-X-e-0);
	\draw[-] (e-H-t-0) -- (t-H-t-0);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(a-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$a$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(b-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$b$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(c-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$c$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(d-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$d$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(e-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$e$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(t-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$t$};



==> figures/reqomp-fig/circuit_w_unqomp.tex <==

\def\tikzRowSepDefault{2mm}
\def\tikzColumnSepDefault{0.5mm}
\def\tikzWireLeftDefault{0.6cm}
\def\tikzWireRightDefault{0.5cm}
\def\tikzWireLabelScaleDefault{0.9}
\def\tikzWireLabelShiftXDefault{-0.1}
\def\tikzWireLabelShiftYDefault{0.17}

\def\tikzRowSep{\tikzRowSepDefault}
\def\tikzColumnSep{\tikzColumnSepDefault}
\def\tikzWireLeft{\tikzWireLeftDefault}
\def\tikzWireRight{\tikzWireRightDefault}
\def\tikzWireLabelScale{\tikzWireLabelScaleDefault}
\def\tikzWireLabelShiftX{\tikzWireLabelShiftXDefault}
\def\tikzWireLabelShiftY{\tikzWireLabelShiftYDefault}

\matrix[row sep=\tikzRowSep,column sep=\tikzColumnSep] (matrix) {
	\node[style=circuit-gate] (u-X-u-0) {$X$}; &
	\node[style=circuit-ctrl] (u-X-v-0) {}; &
	\node[style=circuit-gate] (u-X-u-1) {$X$}; &
	\node[style=circuit-gate] (u-X-u-2) {$X$}; &
	\node[style=circuit-ctrl] (u-H-r-0) {}; &
	\node[style=circuit-gate] (u-X-u-3) {$X$}; &
	\node[style=circuit-gate] (u-X-u-4) {$X$}; &
	\node[style=circuit-ctrl] (u-X-v-1) {}; &
	\node[style=circuit-gate] (u-X-u-5) {$X$}; &
	\node[style=circuit-gate] (u-X-u-6) {$X$}; &
	\node[style=circuit-ctrl] (u-X-v-2) {}; &
	\node[style=circuit-noop] (u-11) {}; &
	\node[style=circuit-ctrl] (u-X-v-3) {}; &
	\node[style=circuit-gate] (u-X-u-7) {$X$}; \\

	\node[style=circuit-noop] (v-0) {}; &
	\node[style=circuit-gate] (v-X-v-0) {$X$}; &
	\node[style=circuit-noop] (v-2) {}; &
	\node[style=circuit-ctrl] (v-X-u-2) {}; &
	\node[style=circuit-noop] (v-4) {}; &
	\node[style=circuit-ctrl] (v-X-u-3) {}; &
	\node[style=circuit-noop] (v-6) {}; &
	\node[style=circuit-gate] (v-X-v-1) {$X$}; &
	\node[style=circuit-noop] (v-8) {}; &
	\node[style=circuit-noop] (v-9) {}; &
	\node[style=circuit-gate] (v-X-v-2) {$X$}; &
	\node[style=circuit-ctrl] (v-H-t-0) {}; &
	\node[style=circuit-gate] (v-X-v-3) {$X$}; &
	\node[style=circuit-noop] (v-13) {}; \\

	\node[style=circuit-noop] (r-0) {}; &
	\node[style=circuit-noop] (r-1) {}; &
	\node[style=circuit-noop] (r-2) {}; &
	\node[style=circuit-noop] (r-3) {}; &
	\node[style=circuit-gate] (r-H-r-0) {$H$}; &
	\node[style=circuit-noop] (r-5) {}; &
	\node[style=circuit-noop] (r-6) {}; &
	\node[style=circuit-noop] (r-7) {}; &
	\node[style=circuit-noop] (r-8) {}; &
	\node[style=circuit-ctrl] (r-X-u-6) {}; &
	\node[style=circuit-noop] (r-10) {}; &
	\node[style=circuit-noop] (r-11) {}; &
	\node[style=circuit-noop] (r-12) {}; &
	\node[style=circuit-ctrl] (r-X-u-7) {}; \\

	\node[style=circuit-noop] (t-0) {}; &
	\node[style=circuit-noop] (t-1) {}; &
	\node[style=circuit-noop] (t-2) {}; &
	\node[style=circuit-noop] (t-3) {}; &
	\node[style=circuit-noop] (t-4) {}; &
	\node[style=circuit-noop] (t-5) {}; &
	\node[style=circuit-noop] (t-6) {}; &
	\node[style=circuit-noop] (t-7) {}; &
	\node[style=circuit-noop] (t-8) {}; &
	\node[style=circuit-noop] (t-9) {}; &
	\node[style=circuit-noop] (t-10) {}; &
	\node[style=circuit-gate] (t-H-t-0) {$H$}; &
	\node[style=circuit-noop] (t-12) {}; &
	\node[style=circuit-noop] (t-13) {}; \\
};
% COORDINATES
% u
\coordinate[left =\tikzWireLeft of u-X-u-0.center] (u-left);
\coordinate[right=\tikzWireRight of u-X-u-7.center] (u-right);

% v
\coordinate[left =\tikzWireLeft of v-0.center] (v-left);
\coordinate[right=\tikzWireRight of v-13.center] (v-right);

% r
\coordinate[left =\tikzWireLeft of r-0.center] (r-left);
\coordinate[right=\tikzWireRight of r-X-u-7.center] (r-right);

% t
\coordinate[left =\tikzWireLeft of t-0.center] (t-left);
\coordinate[right=\tikzWireRight of t-13.center] (t-right);

\begin{scope}[on background layer]
	% wires
	\draw[-] (u-left) -- (u-right);
	\draw[-] (v-left) -- (v-right);
	\draw[-] (r-left) -- (r-right);
	\draw[-] (t-left) -- (t-right);

	% controls
	\draw[-] (u-X-v-0) -- (v-X-v-0);
	\draw[-] (v-X-u-2) -- (u-X-u-2);
	\draw[-] (u-H-r-0) -- (r-H-r-0);
	\draw[-] (v-X-u-3) -- (u-X-u-3);
	\draw[-] (u-X-v-1) -- (v-X-v-1);
	\draw[-] (r-X-u-6) -- (u-X-u-6);
	\draw[-] (u-X-v-2) -- (v-X-v-2);
	\draw[-] (v-H-t-0) -- (t-H-t-0);
	\draw[-] (u-X-v-3) -- (v-X-v-3);
	\draw[-] (r-X-u-7) -- (u-X-u-7);

\end{scope}

% wire labels
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(u-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$u$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(v-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$v$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(r-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$r$};
\node[anchor=base west,scale=\tikzWireLabelScale] at ($(t-left) + (\tikzWireLabelShiftX,\tikzWireLabelShiftY)$) {$t$};



==> figures/reqomp-fig/circuit_w_unqomp_highlights.tex <==

\input{figures/reqomp-fig/circuit_w_unqomp.tex}

\begin{scope}[on background layer]
\draw [split=0.2cm, color= my-full-red, opacity=0.2]
    (u-X-u-0.west) -- % top left
    (u-X-u-1) -- % top left
    (u-X-u-1) -- % top left
    ($(u-X-u-1.west)!0.5!(u-X-u-1.east)$)--
    (u-X-u-0) -- % top left
    cycle;

    \node (ahoriz) at ($(u-X-u-0.west)!0.15!(u-X-u-1.east)$) {};
    \node (avert) at ($(u-X-u-0.south)!0.2!(u-X-u-0.north)$) {};
    \node[color=my-full-red!70, anchor=south west] (a) at (ahoriz |- avert) {$a$};

\draw [split=0.2cm, color= my-full-red, opacity=0.2]
    (u-X-u-4.west) -- % top left
    (u-X-u-5) -- % top left
    (u-X-u-5) -- % top left
    ($(u-X-u-5.west)!0.5!(u-X-u-5.east)$)--
    (u-X-u-4) -- % top left
    cycle;

    \node (ahoriz2) at ($(u-X-u-4.west)!0.15!(u-X-u-5.east)$) {};
    \node[color=my-full-red!70, anchor=south west] (a2) at (ahoriz2 |- avert) {$a$};

\draw [split=0.2cm, color= my-full-green, opacity=0.2]
	(v-X-v-0.west) -- % top left
    (v-X-v-1) -- % top left
    (v-X-v-1) -- % top left
    ($(v-X-v-1.west)!0.5!(v-X-v-1.east)$)--
    (v-X-v-0) -- % top left
    cycle;

	\node (bhoriz) at ($(v-X-v-0.west)!0.1!(v-X-v-1.east)$) {};
	\node (bvert) at ($(v-X-v-0.south)!0.2!(v-X-v-0.north)$) {};
    \node[color=my-full-green!70, anchor=south west] (b) at (bhoriz |- bvert) {$b$};

\draw [split=0.2cm, color= my-full-blue, opacity=0.2]
	(u-X-u-2.west) -- % top left
    (u-X-u-3) -- % top left
    (u-X-u-3) -- % top left
    ($(u-X-u-3.west)!0.5!(u-X-u-3.east)$)--
    (u-X-u-2) -- % top left
    cycle;

	\node (choriz) at ($(u-X-u-2.west)!0.15!(u-X-u-3.east)$) {};
    \node[color=my-full-blue!70, anchor=south west] (c) at (choriz |- avert) {$c$};

\draw [split=0.2cm, color= my-full-orange, opacity=0.2]
	(u-X-u-6.west) -- % top left
    (u-X-u-7) -- % top left
    (u-X-u-7) -- % top left
    ($(u-X-u-7.west)!0.5!(u-X-u-7.east)$)--
    (u-X-u-6) -- % top left
    cycle;

	\node (dhoriz) at ($(u-X-u-6.west)!0.1!(u-X-u-7.east)$) {};
    \node[color=my-full-orange!70, anchor=south west] (d) at (dhoriz |- avert) {$d$};

\draw [split=0.2cm, color= my-full-purple, opacity=0.2]
	(v-X-v-2.west) -- % top left
    (v-X-v-3) -- % top left
    (v-X-v-3) -- % top left
    ($(v-X-v-3.west)!0.5!(v-X-v-3.east)$)--
    (v-X-v-2) -- % top left
    cycle;

	\node (ehoriz) at ($(v-X-v-2.west)!0.15!(v-X-v-3.east)$) {};
    \node[color=my-full-purple!70, anchor=south west] (a2) at (ehoriz |- bvert) {$e$};
\end{scope}



==> headers/lqa/abbreviations.tex <==
% Description: This file defines commands for common abbreviations
%
% Usage: \input{headers/lqa/abbreviations}

% The Backslash between `.` and ` ` is needed to ensure the white-space is an
% inter-word space, not a inter-sentence space.
%
% Details:
% - https://tex.stackexchange.com/questions/2229/is-a-period-after-an-abbreviation-the-same-as-an-end-of-sentence-period
% - https://stackoverflow.com/questions/2024338/latex-sometimes-puts-too-much-or-too-little-space-after-periods/2024341

\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }
\newcommand{\etc}{etc.}
\newcommand{\cp}{{cp.\ }}
\newcommand{\nth}[1]{\ensuremath{#1^\text{th}}}
\newcommand{\wrt}{{w.r.t.\ }}

==> headers/lqa/csvsimple.tex <==
% Description: This file enables displaying csv tables
%
% Usage: \input{headers/lqa/csvsimple}

\usepackage{csvsimple}

% EXAMPLE USAGE

% \begin{table}
% 	\begin{tabular}{ll}
% 		A & B \\
% 		\hline
% 		\csvreader[%
% 			head to column names,
% 			late after line=\\,
% 			separator=semicolon
% 		]{algorithms.csv}{}{%
% 			\a & \b
% 		}
% 	\end{tabular}
% 	\caption{Caption.}
% 	\label{tab:label}
% \end{table}

==> headers/lqa/headings.tex <==
% Description: This file defines headings
%
% Usage: \input{headers/lqa/headings}

\makeatletter

% for IEEE:
% replace trailing : by trailing .
\def\@IEEEsectpunct{.\ }

% Definition for paragraphs, handling spacing correctly
% https://tex.stackexchange.com/questions/31780/where-can-i-find-help-files-or-documentation-for-commands-like-startsection-fo
% http://joshua.smcvt.edu/latex2e/bs-at-startsection.html
\def\mypara{\@startsection%
	{paragraph}% 
	{4}% level
	{0\parindent}% indent
	{0.6ex plus 0.1ex minus 0.1ex}% beforeskip
	{0ex}% afterskip
	{\normalfont\normalsize\bfseries}% style
	*% do not number
}%

\makeatother

\newcommand{\para}[1]{\mypara{#1. }}

% Alternatively: Define \para in terms of \paragraph
% \newcommand{\para}[1]{\paragraph{#1.}}

==> headers/lqa/subfigures.tex <==
% Description: This file introduces a subfigure which correctly aligns
% captions
%
% Usage:
% - \input{headers/lqa/subfigures}
% - You may need to comment out the usepackage command below in case of
%   conflicts

% EXAMPLE USAGE:
%
% \begin{figure}
% 	\centering
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 1
% 	}{Caption of subfigure\label{fig:subfig1}}
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 2
% 	}{Caption of subfigure\label{fig:subfig2}}
% 	\caption{An example of subfigures.}
% 	\label{fig:subfigures}
% \end{figure}

%%%%%%%%%%%%%%
% USEPACKAGE %
%%%%%%%%%%%%%%
\usepackage{subcaption}

%%%%%%%%%%%
% COMMAND %
%%%%%%%%%%%

\newcommand{\mysubfigure}[3][\linewidth]{\subcaptionbox{#3}[#1]{
	\begin{minipage}{#1}
		% uses minipage to prevent unexpected interactions,
		% e.g., for align
		#2
	\end{minipage}
}}

